An Integrative Analysis of the Rich Planetary System of the Nearby Star e Eridani: Ideal Targets For Exoplanet Imaging and Biosignature Searches

e Eridani, the fifth-closest Sun-like star, hosts at least three planets and could possibly harbor more. However, the veracity of the planet candidates in the system and its full planetary architecture remain unknown. Here we analyze the planetary architecture of e Eridani via DYNAMITE, a method providing an integrative assessment of the system architecture (and possibly yet-undetected planets) by combining statistical, exoplanet-population level knowledge with incomplete but specific information available on the system. DYNAMITE predicts the most likely location of an additional planet in the system based on the Kepler population demographic information from more than 2000 planets. Additionally, we analyze the dynamical stability of e Eridani system via N-body simulations. Our DYNAMITE and dynamical stability analyses provide support for planet candidates g, c, and f, and also predict one additional planet candidate with an orbital period between 549 -- 733 days, in the habitable zone of the system. We find that planet candidate f, if it exists, would also lie in the habitable zone. Our dynamical stability analysis also shows that the e Eridani planetary eccentricities, as reported, do not allow for a stable system, suggesting that they are lower. We introduce a new statistical approach for estimating the equilibrium and surface temperatures of exoplanets, based on a prior on the planetary albedo distribution. e Eridani is a rich planetary system with a possibility of containing two potentially habitable planets, and its vicinity to our Solar System makes it an important target for future imaging studies and biosignature searches.

==> Final_report.tex <==
We again thank the referee for their comments that improved our manuscript and appreciate the straightforward and precise manner in which this review was performed.

=================[ REFEREE'S COMMENT]========================
Line 137: Is this sentence missing the ending? The following sentence also seems to have the parenthesis around the wrong phrases. This is an important part of the discussion of caveats so I suggest the authors revise this section so that it is clearer.
-----------[ AUTHORS' RESPONSE]========================
We thank the referee for bringing this to our attention. We have revised the specified paragraph.

=================[ REFEREE'S COMMENT]========================
Line 927: You might also want to point out that the Pluto-Neptune system is stable because of the 3:2 resonance. As these planets are likely non-resonant, this is unlikely to be the case.
-----------[ AUTHORS' RESPONSE]========================
We agree with the referee and now state the 3:2 resonance stability in our manuscript. 

=================[ REFEREE'S COMMENT]========================
I understand that the authors have removed some text in the final sections to make the paper less repetitive and verbose. I still think it is very repetitive and could be shortened substantially without loss of meaning. I will not hold up acceptance for an additional round of revisions in this manner, but I strongly encourage the authors to remove substantial sections of text the largely reiterate information that has already been described in detail (e.g.: what is analyzed).
The new conclusions section is an outstanding improvement.
-----------[ AUTHORS' RESPONSE]========================
While we do agree with the referee that some parts of the manuscript reiterate information. We believe that it is done in a way to highlight the important parts for discussion and therefore have not substantially shortened the paper. Still we thank the referee for this comment. 

=================[ REFEREE'S COMMENT]========================
Line 1182: I would cite P11 and F17 again here.
-----------[ AUTHORS' RESPONSE]========================
We agree with the reviewer that the previous works should be specified. Consequently we have cited these works. 

==> Report_23_January.tex <==
We thank the reviewer for the careful review and concrete comments on how to further improve our manuscript.
We considered and implemented every single comments and suggestion by the referee, which improved our manuscript.

There is only one more major change that this work resulted in: Following the referee's suggestion and concerns about the best-fit eccentricities from the Feng et al. 2017 study, we implemented a comprehensive dynamical stability analysis of the system. We now discuss the constraints this analysis identified on the planetary eccentricities and we adjusted the discussion and results section of our manuscript to be fully consistent with those considerations.

In the following, we will explain how we addressed each of the reviewer's comments.

=================[ REFEREE'S COMMENT]========================
I have reviewed the manuscript "An Integrative Analysis of the Rich Planetary System of the Nearby Sun-like Star e Eridani: Ideal Targets for Exoplanet Imaging and Biosignature Searches" by Basant et al. I also read the previous review correspondence. In this paper, the authors use a model "DYNAMITE" (developed by the co-authors) to study the planetary system around e Eridani. Two previous RV studies have confirmed the existence of 3 planets in the system, and provided weak data for 3 additional signals. The goal of this paper is to use a model based in exoplanet demographics and dynamical stability criteria to assess how likely it is that the other 3 signals are genuine (and if the system might host other planets). The authors' model favors all 3 unconfirmed planets being genuine, and also predicts a 7th planet exterior to the known system residing in the habitable zone. The paper then invokes a simple model for determining the surface temperature of the planets to argue that the 6th and 7th planets might be habitable, and are ideal targets for future direct imagining characterization given the proximity of the system to the Sun.

It is my understanding that the first review of this paper was quite critical. While I see that the authors have made substantial modifications to satisfy the concerns of that reviewer, unfortunately, my review is rather critical as well (though I am not as skeptical of the study's overall merits). The first review points out that a predictive model motivated by population demographics (rather than one utilizing MMRs, TTVs, etc.) is not the right tool to use for inferring the existence of actual planets. I agree with this. However, in my opinion that doesn't preclude a robust investigation of the hypothetical from being scientifically worthwhile and noteworthy (many groups have investigated the implications of extra planets existing in other systems such as TRAPPIST, eg: Kral et al., 2018 and Raymond et al. 2021). If framed in the correct manner, a study such as this one is still useful in my opinion. Unfortunately, in its current form, I do not think this paper is worthy of publication as this category of investigation. I am happy to review a substantially revised version of the study as I think the overall content is interesting and will be a noteworthy contribution to the current literature if my (many) concerns are addressed.

In general, I don't think the authors adequately articulate their points, and I am not convinced by the arguments made about the DYNAMITE model's merits. More superficially, the paper could benefit from significant editing for grammar, run-on sentences and overall length. In its current form it is a very long read, and quite repetitive. I believe the manuscript would be much more impactful and interesting to read if condensed significantly. My major issues with the substance of the work center around the eccentricities of the planets predicted in the RV analysis of Feng et al. 2017, the apparently unsupported claim that the author's model incorporates a robust collection of constraints from dynamical stability and formation models, the seemingly arbitrary outer orbital period of 2 years considered by the model, and the lack of a discussion of model limitations in the text. I have many comments that are listed in chronological order, and have annotated comments I see as major issues with the *** symbol. Many of these comments are similar in that they relate back with the aforementioned four major issues, so the total number of *** symbols is much more than the number of real major issues I see with the paper.

-----------[ AUTHORS' RESPONSE]========================
We thank the referee for their multiple excellent comments on the manuscript. The referee report included 45 comments. Over the last 2 months, we considered each comment carefully and implemented all of the comments.
In our response below, we discuss how we implemented the changes advised by the reviewer. We use the bold font (\edit1) to identify the changes that have been made in the manuscript. There is also a small number of comments in which we did not agree with the referee. 

=================[ REFEREE'S COMMENT]========================
Line 11: "via DYNAMITE, providing"... would be clearer as "via DYNAMITE, a code which provides an integrative...."

-----------[ AUTHORS' RESPONSE]========================
We agree with the referee and have replaced the phrase "via DYNAMITE, providing" with "via DYNAMITE, a method providing an integrative...".

=================[ REFEREE'S COMMENT]========================
The use of manuscript-specific acronyms (H[d]-PxP-1) should be removed from the abstract.

-----------[ AUTHORS' RESPONSE]========================
We removed this acronym from the abstract.  

=================[ REFEREE'S COMMENT]========================
The discussion of the potential surface temperatures of the exoplanets takes up half of the abstract but is, in my opinion, more of a minor aspect of the paper as currently written. It would be useful to condense this material to just a sentence or so in the abstract, and use the additional space to provide more details on what goes into the model (i.e.: what exoplanet statistics is it based off of).

-----------[ AUTHORS' RESPONSE]========================
We followed the referee's suggestion and updated the abstract significantly. We now also include the information about eccentricity analysis and results in the abstract.

=================[ REFEREE'S COMMENT]========================
Line 35: Citation not provided

-----------[ AUTHORS' RESPONSE]========================
We appreciate the referee to bring this to our attention. We have now updated the citation in the manuscript. 

=================[ REFEREE'S COMMENT]========================
***The authors mention on line 41 that "the emerging body of information on exoplanet demographics and on planet formation and evolution, can be combined to improve the understanding of individual planetary systems." It is unclear to me how formation models are used at all in the analysis. It would be interesting to use eccentricity and inclination distributions from formation models, or even planet compositions that come from population synthesis models, in the analysis. To my understanding, this is not done.

-----------[ AUTHORS' RESPONSE]========================
We thank the referee for pointing out that this sentence may be misleading. The referee is indeed correct: No formation models are currently integrated into our analysis. We rephrased the sentence to clarify that we are describing a future possibility and not an already implemented source of information.


=================[ REFEREE'S COMMENT]========================
***Line 66: Here, the authors introduce the 6 planet model of the system proposed in Feng et al. 2017 that will be used throughout the paper. Feng's best fit has fairly large eccentricities for most of the planets (particularly b, d and e). In fact, as the authors point out, it is easy to see that some of the planets in this solution are on crossing orbits. For instance, the apocenter of the 89 day signal would be .45 au, and the pericenter of the 147 day signal is at .36 au. Feng acknowledges that the system is not dynamically stable, and notes that instrumental noise and fitting bias might be the cause of the high eccentricities. Unless there is newer work on the system that shows a good fit at low-e, I see this as a major weakness of any paper like this one building on Feng's work. At a minimum, the authors need to discuss this (i.e.: make a convincing argument as to why Feng's eccentricities are over estimated rather than reiterating what is said in that paper), and also perform dynamical simulations to determine the maximum eccentricities which allow a six planet configuration to remain stable on ~Gyr timescales (I suspect this is something in the 0.05-0.1 range). If the authors cannot make a convincing case that the such a system could be stable within Feng's error bars for e, I don't think it is justified to report the authors findings as "additional evidence for potential candidates."

-----------[ AUTHORS' RESPONSE]========================
We agree that this is an important aspect of the dataset.  As the referee suggested, we now include a detailed assessment of the dynamical stability of the planetary system as a function of the planetary eccentricities. Specifically, we ran 4 different simulations of two different planetary architectures -- the 3 planet system with planets b, d, and e and the six planet system with planets g, b, c, d, e, and f. For both of these system architectures, we ran two sets of simulations: the first had a normal eccentricity distribution (corresponding to the eccentricities from the best-fit orbital solutions in Feng et al. 2017), while the second set used a lognormal eccentricity distribution, following He et al. 2020. This latter setup represents the eccentricity distribution of typical planetary systems (i.e., represents a case where we do not rely on the eccentricity fits from Feng et al. 2017).

This analysis brought clear results:
For the system with b, d, and e as genuine planets, we found that out of 1000 iterations with the parameters from Feng et al. 2017 (a Normal distribution), only 1.2 \% resulted in the planetary system being dynamically stable. With lognormal parameters from He et al 2020, 1.7 \% out of 1000 iterations were unstable. 

In contrast, including all the six planet and planet candidates, the Feng et al. 2020 parameters resulted in only one stable configuration out of 1000 iterations, while the lognormal eccentricity distribution resulted in roughly 1.1 \% out of 1000 iterations as unstable. 

Our results demonstrate that the referee is correct in their assessment that the dynamical stability of this system depends on the assumed eccentricities.  Our results advocate that it is highly unlikely for the e Eridani planetary system to be stable with the eccentricity values proposed by Feng et al. 2017 and the planets in the system indeed have to have lower eccentricity. (A possibility Feng et al. also identified) 

Given the above, we made the following revisions in the manuscript:

(1) We describe the analysis in subsection 3.4.

(2) The numerical experiment results are discussed in subsection 4.3.

(3) In subsection 5.2, we discuss that the eccentricity as reported in Feng et al. 2017 paper are unlikely to result in a stable system and that, for the system to be stable, the planets should indeed have lower eccentricities. 

Given this context, we agree with the referee that our results for additional planets should be presented as additional evidence only under the assumption that the planets in e Eridani system have lower eccentricities than reported. We also provide constraints on the eccentricity of all the planets combined in a 3 planets as well as a 6 planet system. 

We thank the referee again for their comment and we feel that the above changes fully address this aspect of the manuscript.

We also note that if the estimates for eccentricities are updated in the future, then our analyses must be repeated. In addition to this, we also acknowledge in the manuscript that our results from DYNAMITE analysis only remain valid if the planets in the e Eridani system have lower eccentricities than reported in previous works. 

=================[ REFEREE'S COMMENT]========================
The paragraph beginning on line 79 needs to be edited for grammar, clarity and brevity. Several of the sentences are confusing to understand, DYNAMITE is introduced twice, etc.

-----------[ AUTHORS' RESPONSE]========================
We revised this paragraph significantly.

=================[ REFEREE'S COMMENT]========================
***Two paragraphs beginning on line 111 and 145. This is all interesting, but to me it is not that convincing. I just see this as predicting that a planet can be there if one can fit. What does the model predict should be in the asteroid belt of the solar system if you give it the known 8 planets? I would guess it would predict a planet should be there. What about interior to Mercury as in the appendix figure? Or what if you took Mercury out, would it predict multiple planets interior to Venus? I'd think it would since that's the way most exoplanet systems look. My point is that it would be more informative to give a couple sentences on how the model has been tested with some real systems minus a planet, and then spend more time talking about the limitations of the methodology.

-----------[ AUTHORS' RESPONSE]========================
We thank the referee for these suggestions. We revised the relevant paragraphs to provide additional examples for our analysis and to highlight some of limitations.

In addition to these examples, we also included in the introduction, a brief summary of the limitations of our analysis.
Specifically, we stress that our analysis is based on available data, i.e., it is not clear to what extent it can be extrapolated in the following dimensions: (a) planet radius smaller than ~0.5x Earth value and larger than 4x Earth value; (b) beyond ~700 day-long periods; (c) non-planetary objects, such as asteroid belts. Finally, our predictions are more likely to be correct for typical planetary systems and less likely to be correct for atypical or exceptional systems.

These points specifically address the referee's questions about Mercury (a planet with a size too low for the range we considered here, and orbiting in an unusual inner planetary system, e.g., Mulders et al. 2018). It also addressed the question of the asteroid belt: the asteroid belt, in fact, is widely identified as the most likely location for an additional planet in the Solar System, but it is thought that planet formation did not conclude there, perhaps due to the presence of Jupiter. 

In conclusion, we followed the referee's suggestion by adding more specific examples of planet recovery tests and highlighting the parameter range within our model should be expected (and was demonstrated) to be reliable.

=================[ REFEREE'S COMMENT]========================
Line 140-144. Doesn't this just repeat what was already elaborated on in the paragraph? 

-----------[ AUTHORS' RESPONSE]========================
We agree that this was repetitive and have removed this part from the paragraph. 

=================[ REFEREE'S COMMENT]========================
Line 186: Remove. This was just stated in the previous paragraph. 

-----------[ AUTHORS' RESPONSE]========================
We removed the said line.  

=================[ REFEREE'S COMMENT]========================
Line 233: "potential of its planets to be habitable" -> "potential habitability of the system" ?

-----------[ AUTHORS' RESPONSE]========================
We agree with the reviewer about the said syntactical change and implemented it. 

=================[ REFEREE'S COMMENT]========================
Line 241: m sin(i) ?

-----------[ AUTHORS' RESPONSE]========================
We have revised this point and thank the referee for bringing it to our attention.

=================[ REFEREE'S COMMENT]========================
Line 265: Also cite Izidoro et al. 2017 for an explanation of the under-abundance of resonant super-Earths compared to the predictions of formation models.

-----------[ AUTHORS' RESPONSE]========================

Given the changes in the handling and discussion of the eccentricities (shift from formation/evolution models to N-body dynamical stability assessment), we removed this paragraph.


=================[ REFEREE'S COMMENT]========================
Line 280: citep->citet

-----------[ AUTHORS' RESPONSE]========================
We appreciate the referee pointing this out and have implemented this change. 

=================[ REFEREE'S COMMENT]========================
Same sentence: This is not a correct summary of the Laskar paper. Angular momentum is conserved in a planetary system. Laskar 1997 showed that angular momentum can be exchanged between planets, yes (in particular, leakage to Jupiter via coupling with the g5 secular resonance), however, in the solar system, this does not zero eccentricities over long periods of time (in fact, it is still challenging to replicate the solar system's terrestrial planets' low eccentricities in formation models, e.g.: Chambers 2001, Clement et al. 2019). Low eccentricities of course come out of instabilities (e.g.: ejections or collisions as the authors mention), but more often the result is high eccentricities. I think that it is more likely that the eccentricities of known exoplanets (and the solar system's terrestrial planets) are low by virtue of having formed while gas was still present in the system (again, see Izidoro et al. 2017).

-----------[ AUTHORS' RESPONSE]========================
We thank the referee for this insightful comment.

Given our now-extended analysis of the possible range of eccentricities that are consistent with the planetary system's stability, the Laskar reference and the other, related references on the theoretical assessment of angular momentum distribution and evolution in planetary systems is no longer important for our analysis. Therefore, in order to streamline the text as recommended by the referee, we eliminated the relevant paragraph, also addressing the referee's comment.


=================[ REFEREE'S COMMENT]========================
***Line 298: I do not see how reducing the eccentricity of d provides more support for existence of c. This sentence should be removed.

-----------[ AUTHORS' RESPONSE]========================
We agree with the referee that citing Feng et al. 2017 for their statement does not provides strong evidence. We now include our own analysis for constraining the eccentricities of the planets in the e Eridani system and removed the mentioned statement.  

=================[ REFEREE'S COMMENT]========================
Line 330: I don't think its necessary to summarize Kopparapu et al. 2013,2014 in this level of detail here as these relations are commonly used in exoplanet papers. The authors can keep this level of detail if they wish, but I think the paper could be abbreviated (and thus be more readable and impactful) if this was replaced with a single sentence to the effect of "We use relations from Kopparapu et al. (2013,2014) to calculate the inner and outer habitable zone edge for a 5 M_earth planet and 1 M_earth planet around e Eridani" 

-----------[ AUTHORS' RESPONSE]========================
We agree with the reviewer and decided to replace to extensive summary of Kopparapu et al. 2013, 2014 with a single sentence.

=================[ REFEREE'S COMMENT]========================
***Line 395: Reference? Chambers et al. 1996 perhaps? Is eccentricity not factored in to this? This seems like a very simplistic criterion as there are many more sophisticated ways of looking at stability then just mutual Hill radii (see, for example, Tamayo et al. 2021). This relates back to my comment about how the authors claim that their model robustly uses constraints from evolution and formation models, when in reality it seems that they just use mutual Hill radii.

-----------[ AUTHORS' RESPONSE]========================
We thank the reviewer for this comment and agree that additional ways to consider stability (including eccentricity) are helpful. We have adjusted our analysis and described that change in the text.

=================[ REFEREE'S COMMENT]========================
First paragraph of 3.2 is also redundant as this was all mentioned in the introduction. 

-----------[ AUTHORS' RESPONSE]========================
We agree with the reviewer that the said paragraph is redundant. We have removed the paragraph from the section. 

=================[ REFEREE'S COMMENT]========================
Line 481: "A general property of dynamically packed systems." What is meant by this? Could the authors provide a reference here?

-----------[ AUTHORS' RESPONSE]========================
We thank the referee for bringing this to our attention and we decided to remove the parenthetical sentence from the manuscript.

=================[ REFEREE'S COMMENT]========================
Paragraph beginning on line 509 is also redundant and could be removed in my opinion.

-----------[ AUTHORS' RESPONSE]========================
We agree with the reviewer and decided to remove the said paragraph. 

=================[ REFEREE'S COMMENT]========================
***Line 528: This also relates back to my comment about how the authors' model does not seem to be motivated by dynamics or formation models as advertised. Most all formation models will predict low mutual inclinations between the planets, so I don't see how this is motivated by formation models. It would be straight forward to use the results of real formation models in the literature as input distributions for the model e/i. This seems like a missed opportunity to me. Am I missing something?

-----------[ AUTHORS' RESPONSE]========================
As clarified above, we are indeed not using planet formation models in the current paper. We agree with the referee for the promise of integrating predictions from planet formation models and we have ongoing projects to accomplish this in the near future.

=================[ REFEREE'S COMMENT]========================
***Line 544: Is the distribution of He et al. 2019 really the right one to use for a single system, particularly given the tendency of neighboring planets in Kepler systems to have similar masses and radii (Millholland et al. 2017)?

-----------[ AUTHORS' RESPONSE]========================
We thank the referee for bringing this to our attention. In general, we agree that there is a tendency for neighboring planets in Kepler systems to have similar masses and radii, but we also know that not every planet is exactly the same size, so we feel that using a Lognormal distribution that is fit to the planets in the system provides the best distribution.

=================[ REFEREE'S COMMENT]========================
Line 578: In the following text?

-----------[ AUTHORS' RESPONSE]========================
We thank the referee for pointing this to us. We have revised the sentence. 

=================[ REFEREE'S COMMENT]========================
Section 3.3: Similar to my previous comments on brevity, this whole section is a very lengthy way of saying that you calculate the equilibrium temperature, assume an albedo (with some discussion about greenhouse), and calculate a surface temperature. The temperature model is simple, and this is fine and a useful addition to the paper. However the text makes it seem like the model is more complex than it is, which is confusing to the reader (I think this might have led to some confusion in the original review).

-----------[ AUTHORS' RESPONSE]========================
We thank the referee for their comment. We agree that the mentioned section was long, which created confusion. We have now significantly revised section 3.3 in the manuscript. 

=================[ REFEREE'S COMMENT]========================
Most of the first first paragraph of 4.1 is redundant and could be removed.

-----------[ AUTHORS' RESPONSE]========================
We agree with the referee and removed first paragraph of subsection 4.1.

=================[ REFEREE'S COMMENT]========================
Line 761: Is this sentence saying that the distribution of potential orbital periods of the outermost planet is wider than that of other predicted planets since DYNAMITE only has one neighboring planet to use to constrain the orbit? Something like that might be clearer.

-----------[ AUTHORS' RESPONSE]========================
We thank the referee for their comment and revised the said sentence.

=================[ REFEREE'S COMMENT]========================
Same section: "genuine planet nature of planet candidate f:" overly verbose and grammatically awkward to me (there are multiple instances of this verbiage throughout the paper). Maybe just "planet candidate f's existence"?

-----------[ AUTHORS' RESPONSE]========================
We agree with the reviewer and revised the mentioned phrase. 

=================[ REFEREE'S COMMENT]========================
***Hypothesis c/d discussion in 4.1, and also 5.3: OK, so the model predicts a planet outside of the current system. This needs some justification beyond being "based on robust statistics from Kepler." As mentioned by the first reviewer, the presence of a planet can be directly inferred dynamically via secular perturbations on the orbit of another planet (i.e.: the discovery of Neptune), orbital distributions of small bodies (i.e.: the current Planet X hypothesis), MMR chains (i.e.: predictions for other TRAPPIST planets). This is not what is done here. This is fine as long as it is put in the appropriate context, which I don't think is done in the current submission. I also don't think the model (as described) is a sophisticated way of looking at the problem. As I understand it (I could be wrong here), the model basically assumes that planets SHOULD exist out to P=2 years (section 3.1; bullet 2) because the more distant Kepler planets have P=2 years. Is this weighted by the total number of planets found out that far? On the one hand, we are biased against detecting further planets, so many Kepler systems might host undetected, further out planets. On the other hand, how many compact systems with multiple 10-100 day orbits have more distant companions? I understand it is probably difficult to build this into a model, but there are also plenty of planet formation population synthesis models out there that could be used as input distributions, and one could envision a way to build a constraint into the monte carlo routine that looks at the total number of planets in known systems or r_inner_planet-r_outer_planet compared to known systems. It would be great to see the authors build a more sophisticated model in this parameter. However, at a minimum, they need to discuss all of these caveats and explain to the reader what is physically making the model predict a planet outside of the known system.

-----------[ AUTHORS' RESPONSE]========================
We thank the referee for this detailed comment and will address it both here and in the text. DYNAMITE only assumes the currently known planets in the system along with the statistical model distributions from the Kepler population as its input data. It then provides a prediction based on what is the most likely place to find one additional planet in the system, if another planet were to exist. When the system has little probability of finding another planet interior to the outermost known planet (i.e., likely dynamically packed), then the most likely place to find an additional planet would be to extend the system out beyond the outermost known planet. In short, this prediction from the model is completely in line with what is expected from general considerations of dynamical stability and exoplanet demographics.

=================[ REFEREE'S COMMENT]========================
"the inner peak is constrained by the innermost known planet as well as the broken power law on the period of the first planet from the orbital period model:" unclear, consider revising.

-----------[ AUTHORS' RESPONSE]========================
We agree with the referee that this specific sentence was unclear. Consequently, we revised the sentence in the manuscript. 

=================[ REFEREE'S COMMENT]========================
Line 823: "likely not to transit" -> "likely not transiting" ? 

-----------[ AUTHORS' RESPONSE]========================
We appreciate the referee's comment and have changed the mentioned phrase. 

=================[ REFEREE'S COMMENT]========================
Figure 2: Why is "Period Ratios" in the legend and in bold? It is clear from the x axis that orbital period is plotted.

-----------[ AUTHORS' RESPONSE]========================
We thank the reviewer for pointing this out, this means we are using the Period Ratios model for distributing planet periods following the statistical prescription in EPOS (Mulders et al. 2018) as compared to the Clustered Periods model from SysSim (He et al. 2019), as these are the two main planet period models currently utilized by DYNAMITE.

=================[ REFEREE'S COMMENT]========================
Much of 4.2 repeats what is described earlier when introducing the model. All that needs to be here are the results in my opinion. 
-----------[ AUTHORS' RESPONSE]========================
We have significantly revised the mentioned subsection for brevity and clarity. We followed the reviewer's advice to only include the results in this subsection.

=================[ REFEREE'S COMMENT]========================
Lines 912-929: remove, this repeats what has already been stated multiple times in the paper now.

-----------[ AUTHORS' RESPONSE]========================
We agree with the reviewer and removed the mentioned paragraph. 

=================[ REFEREE'S COMMENT]========================
5.1-5.3: These sections should also be removed as they repeat what was already stated in the results and methods sections. This is where the authors should make a case for why these planets should exist by expanding on 5.4 in light of my other comments. i.e.: talk about limitations of their model, and about what underlying assumptions are the predictions most sensitive to.

-----------[ AUTHORS' RESPONSE]========================
Following the referee's suggestion, we completely removed the subsections 5.1-5.3. We now discuss the results from our stability analysis and talk about the limitations of the model.

=================[ REFEREE'S COMMENT]========================
***Line 1013: Where is this shown that the results are insensitive to small-moderate changes in the orbital parameters? Did the authors run additional models with different eccentricities? What happens if you assume Feng's eccentricities of ~0.05-0.2? I don't think this statement is justified in the paper.

-----------[ AUTHORS' RESPONSE]========================
We thank the referee for pointing this out. We now included a comprehensive dynamical stability analysis that addresses these points. Please see Section 3.4 for the eccentricity analysis description, 4.3 for the results of eccentricity constraints, and 5.2 for the discussion on eccentricity analysis.   

=================[ REFEREE'S COMMENT]========================
***Line 1019: "not consistent with current orbital fits:" Don't Feng's fits give eccentric orbits? The more interesting question is what happens when you assume those eccentricities instead of zero.

-----------[ AUTHORS' RESPONSE]========================
We now included a comprehensive dynamical stability analysis that addresses these points. Please see Section 3.4 for the eccentricity analysis description, 4.3 for the results of eccentricity constraints, and 5.2 for the discussion on eccentricity analysis.   

=================[ REFEREE'S COMMENT]========================
The first 4 paragraphs of section 6 mostly repeat what has already been stated.

-----------[ AUTHORS' RESPONSE]========================
We significantly revised this section of the manuscript. 

=================[ REFEREE'S COMMENT]========================
Line 1109: "not habitable for life as we know it:" Reference?

-----------[ AUTHORS' RESPONSE]========================
We have now updated this line in the manuscript. 


=================[ REFEREE'S COMMENT]========================
***Line 1134: OK, was the algorithm "told" about Jupiter here?

-----------[ AUTHORS' RESPONSE]========================
We did not include Jupiter in our analysis on the inner Solar system as we ran the simulations for planets with period 2 years or less only. We now clarify specifically in the manuscript that we do not include Jupiter in our analysis. 

=================[ REFEREE'S COMMENT]========================
Line 1064: "too weak gravity to hold an atmosphere" -> "insufficient surface gravity for atmospheric retention" ? 
-----------[ AUTHORS' RESPONSE]========================
We appreciate the proposed change and have revised the mentioned phrase. 

=================[ REFEREE'S COMMENT]========================
I think the list of bullets in the conclusions would be better summarized in a nice, well-written paragraph that says their model correctly predicts the candidates when given no information on them, and predicts an additional planet in the HZ with a surface temp that might be hospitable to life. Then an additional paragraph summarizing the limitations as discussed in my previous comments.

-----------[ AUTHORS' RESPONSE]========================
We thank the referee for their comment. Implementing referee's suggestion, we revised the summary section significantly and now discuss all the results briefly in paragraphs.

==> Response_to_reviewer.tex <==
The authors use a population synthesis model developed in Dietrich & Apai (2020) to probe the orbital period space of e Eridani for potential planets. The model combines occurrence rate estimates for exoplanet orbital period, radius, and inclination with the dynamical spacing parameter for multiple planet systems (Delta_c = 8). The goal of the paper is to evaluate a series of hypotheses concerning the system architecture using population synthesis, where the returned likelihood is interpreted as whether a planet exists at a particular orbital period. The authors claim that all six planets are genuine and a possible seventh planet lurks within the host star's habitable zone. The authors estimate the surface temperature using the variance in albedo of solar system objects and evaluate some scenarios with a basic climate model. Finally, the authors claim that e Eridani is a good candidate for future study given that it is close, potentially hosts up to seven planets, and some of those planets could be in the habitable zone.

-----------[ AUTHORS' RESPONSE]========================

We appreciate the referee's detailed review and several excellent comments.
The referee report included 121 comments. Over the past three months, we considered each comments carefully and implemented over 92\% of the comments.
These comments have greatly improved the quality of the manuscript and we thank the reviewer for bringing these points to our attention.
There is a small number of comments in which we did not fully agree with the referee (or comments that were addressed through previous changes). 
In our response below, we detail how we address the referee's comments. The revised manuscript uses the AAS macros to identify text that was updated.

=================[ REFEREE'S COMMENT]========================
General Comments:
The authors are confused with the results of their model. Population synthesis (on its own) has an abysmal track record for identifying true systems. The oldest known attempt is the Titius-Bode Law, which use a geometric series to "predict" the locations of successive planets in the solar system. It is true that such a relation correlates well with the planets known at the time, but it lacks a physical basis and eventually breaks down. The same is true for this study. The population synthesis model counts up the ways of placing planets within the system and reveals the location where an object **could** reside. Since the physical or observational evidence is very weak in this system, this is where the authors should stop. 

-----------[ AUTHORS' RESPONSE]========================

We understand that the introduction of the manuscript provided insufficient background to introduce the reader to the methods, which may have led to the referee to fail to understand the method used and the relevance of the results.

For the record, we state that the referee's characterization of our work is fundamentally incorrect and appears to lack objectivity. 

The point in which we agree with the referee is that a more comprehensive introduction of the methods and past results will help readers. Therefore, we revised the introduction to better explain how our approach works. This should clarify that our approach is:
1) Different from the approaches commonly referred to as "population synthesis models".
2) Built by combining statistical analysis of a rich dataset on exoplanets and with robust physical foundations.
3) One with a track record of repeatedly, correctly predicting planet properties. 

We hope that the revised introduction will help the readers and the referee better understand our approach and form an objective opinion.

=================[ REFEREE'S COMMENT]========================
The authors do contribute to the distribution of albedos, but they push forward on shaky ground to make estimates for planets that may or may not exist. Including results from a climate model is also a good idea, but the setup of the climate model is absent. As a result, the sections considering each planet's surface temperature is not reproducible. I cannot recommend the paper for publication and many changes to the methodology are necessary to revise the manuscript into an acceptable form.

-----------[ AUTHORS' RESPONSE]========================

The referee misunderstood the manuscript. No climate model was used or mentioned, thus there is no need to describe the setup of the climate model. 
In response to this comment, we thoroughly reviewed the relevant sections and slightly edited, where necessary, to further clarify the model used for the temperature estimates. Further, we also added a test to show that our approach, when applied to Mars as an example, would predict Mars' orbital period to within 2% and its surface temperature well within the actual range of measured surface temperatures. We included additional discussion of this test and the validity of the model used in the manuscript.

For the temperature estimate, our analysis uses a simple energy balance model, a.k.a. radiative equilibrium model, only modified to include a single-layer semi-transparent absorber layer (representing a weak greenhouse effect). This model is, in fact, captured in two equations, both of which are provided in the manuscript. The few parameters used in these equations (stellar luminosity, planet-star separations, albedo, and absorbing efficiency of the greenhouse layer) are also provided in the manuscript. Our entire approach and the results are documented in the manuscript and are thus reproducible. 

=================[ REFEREE'S COMMENT]========================
Herein, I list the major issues with the paper:

Section 1: 
The introduction is altogether insufficient. It identifies some of the stellar parameters, suggests a few questions (one of which probably can't be answered anyway), and gives an outline. The relevant literature review consists of 3 sentences that refer to previous works of the co-authors. A much more substantial literature review needs to be included similar to the authors previous work (e.g., Dietrich & Apai 2020).

-----------[ AUTHORS' RESPONSE]========================

We agree with the referee that the introduction lacked details on relevant past work.
We extended the introduction to better explain the fundamentals of our analysis and list a number of papers where it was successfully tested and used.

=================[ REFEREE'S COMMENT]========================
In the very beginning, the authors need to give some of the alternate names for e Eridani. Most readers will be unfamiliar with this system as it is overshadowed by epsilon Eridani. Even though it is not the author's intent, many readers will confuse the two systems and realize later that it is a different system than they may have supposed.

-----------[ AUTHORS' RESPONSE]========================

We followed the referee's comment and identify alternate names and point out explicitly that this star is not epsilon Eridani.

=================[ REFEREE'S COMMENT]========================
Section 2:
The section provides much of the tabulated background, but it does not provide a clear roadmap for the reader. The first discussion on stellar parameters seems to miss that e Eridani appears to be on the border of stellar classification schemes. The stellar classification goes into many assumptions for climate models and could significantly alter the author's conclusions.

Section 2.2 provides a background information for the previous observations, but it doesn't lead the reader into why the background is important. There is a paragraph concerning the possibility of an outer disk, but this is not mention elsewhere or whether it will be used as additional evidence for unseen planets. The authors use an assumption for low planetary eccentricity, but there are citations missing for the claim and the assumption is missing context that is known from the solar system (e.g., Laskar 1997 study on angular momentum deficit and meta-stability of the solar system).

-----------[ AUTHORS' RESPONSE]========================

We agree with the referee that e Eridani is near a stellar classification border. We now explicitly mention this in the manuscript. However, the spectral type is not relevant for our study: We are using stellar luminosity (derived from high-precision distance measurements and model atmosphere fits to high-quality spectroscopic observations). We now state this in the manuscript.

We also include context for the importance of previous observations given for this system's planets and debris disk.

We thank the reviewer for pointing out the study by Laskar (1997) and works that build on it. These are indeed relevant to our argument and setup.
We extended the relevant discussion in the manuscript and included the citations.

=================[ REFEREE'S COMMENT]========================
Section 3:
The authors define each of the system architectures as hypotheses. But they do not explore how they are constructed or whether they are unique. There is a wide range of planetary orbits possible interior to or exterior to a multiple planet system. As a result, a planetary orbit could always be found via population synthesis and have a large apparent likelihood, but an infinite number of planets do not exist (i.e., there are no physical penalties in the statistical model). As a result, only Hypothesis H[a] can be seriously tested and additional observational evidence is necessary to confirm planet c (see Hinse et al. 2015 and Orosz et al. 2019 for an example). The remaining hypotheses are speculative at best.

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for pointing out the lack of clarity on how and why the hypotheses are constructed.

We addressed this concern via three steps:
1) We now evaluate all combinations of the candidate planets being genuine or not. Four hypotheses (which we consider the most likely) are kept in the main body of the manuscript, while the rest are placed in the Appendix. Comparison of the results of all these hypothesis shows that the planetary architectures predicted are very similar.

2) We now better explain the approach that leads to the prioritization of the four hypotheses highlighted in the main body of the manuscript. 

3) We also discuss and show that our results are quite insensitive to the order in which planets are placed in the system; therefore, starting from the set of three confirmed planets, it does not really matter in which order the 4th, 5th, and 6th planets are added: the results converge to the same architecture.

On the separate point mentioned above, we agree with the referee that additional data are required to confirm the existence of the candidate planets; however, we point out that the goal of predictions -- such as ours -- is not to confirm planets but to identify a connection between a hypothesis and its potentially testable consequence. 

On another point above ("only Hypothesis H[a] can be seriously tested"): This is simply an incorrect statement. The hypotheses identified produce specific observable signals that can potentially be detected via radial velocity and via direct imaging.

On the other point above: "but an infinite number of planets do not exist (i.e., there are no physical penalties in the statistical model)": 
We believe that the referee misunderstood how our analysis works; hopefully, the revised introduction address their concerns. 

=================[ REFEREE'S COMMENT]========================
The surface temperature assessment provides a lot of detail concerning the surface temperature with the albedo prior, but very little detail regarding the climate model. Readers would have more questions concerning the setup of the climate model because small changes in the initial conditions can lead to very different results (i.e., reproducibility problem). Also, it seems that most of the section can be contextualized to the expectation that T_surf \propto (1-A_B)^(1/4)/P^(1/3), where P is the orbital period. The main trend is determined by orbital period and the variance along the trend is given by the assumptions on the albedo prior.

-----------[ AUTHORS' RESPONSE]========================

The referee seems to assume that there is a climate model for which no explanation was provided, but this is not the case. Our model consists of a single-layer leaky greenhouse prescription, which is a simple and relatively common modification of the radiative equilibrium (energy balance) models. The section does include the specific equations used (Eqs. 1 and 2), which provide sufficient information for a completely reproducible solution. All data are provided. 

This also addresses the referee's second comment: Indeed, the behavior of the model is what one would expect from the radiative equilibrium-based prescription. This is a consequence of the fact that our model is a modification on the radiative equilibrium model.

Nevertheless, we reviewed carefully the text to make sure that there is no misleading mention of a climate model.

=================[ REFEREE'S COMMENT]========================
Section 4
Figure 1 is a summary of the logical conclusions given the hypotheses, which are described in the text. It is framed as results, which is an overstatement.
Another major problem is that the Feng+ 2017 provides the minimum mass measurements for only the 6 planet model and the authors use these values in their Hypotheses H[a]-H[c] without re-evaluating the RV solution. This is necessary because the best-fit mass for planets b, d, and e are likely different in the 3 planet solution as compared to the 6 planet solution. Moreover, the best-fit eccentricity of the planets will also increase, which can drastically affect the results presented by the authors. For example, a higher eccentricity for planet b or d will reduce the allowed period space for planet c.
-----------[ AUTHORS' RESPONSE]========================

As requested, in Figure 1 we changed the word "results" to "predictions".

We appreciate the referee's point about the potential importance of re-evaluating the RV solutions for different number of planets. The referee highlights that the best-fit mass for planets may be different depending on how many planets are included in the RV fit.  

We addressed this point in a new subsection (5.4).

=================[ REFEREE'S COMMENT]========================
The results for the possible surface temperatures needs clarified and contextualized. The first estimates are for the equilibrium temperatures, where the second set are determined using the climate model. It is unclear that the precision in the error bar is reasonable for either set. There are many assumptions that go into the either set that go unstated. The leaky greenhouse model needs to be described in more detail so that readers are informed of what assumptions are made about the atmosphere and resultant greenhouse warming. The results are provided in the text separately, but how do they compare to each other? How do they compare with an even simpler model using the Stefan-Boltzmann Law (i.e., how much does the albedo contribute?)?

-----------[ AUTHORS' RESPONSE]========================

We now expanded and further clarified the relevant section, and also included an example (Mars) for how the model works. Nevertheless, we point out that the referee incorrectly assumes that there are "many assumptions [..] that go unstated". This is not the case, as explained above; we use the model that is described in the text, and that description is complete. There is no separate, detailed climate model with hidden assumptions. 

=================[ REFEREE'S COMMENT]========================
The authors use Hypothesis H[d] to infer the existence of an exterior planet at 611 days, when they only show that the current measurements allow for an additional planet. There is no empirical evidence to support their predicted planet. Previous studies (Nesvorny+ 2013, Hinse+ 2015, even the discovery of Neptune) predicted an additional planet guided by relevant physical phenomena (typically mean motion resonances).

-----------[ AUTHORS' RESPONSE]========================

We agree with the referee that our analysis is not based on the same type of data that was used for the discovery of Neptune. We also agree that there is no direct evidence for the existence of a planet at a period of approximately 611 days in this specific system. 

However, we shall point out that the referee's general argument above does not apply to our work:

Contrary to the referee's statement, we did not "claim to infer" the existence of a planet -- instead, we formulated a hypothesis and presented a prediction from that hypothesis. 

In this process, the availability of  "empirical evidence" is not a requirement for the validity or value of predictions.

For example, according to the Oxford English Dictionary, a *hypothesis* is "A proposition or principle put forth or stated (without any reference to its correspondence with fact) merely as a basis for reasoning or argument, or as a premiss from which to draw a conclusion; a supposition. "
In the scientific method, hypotheses are tested by experimental assessment of the validity of predictions that are made from the hypothesis. 

Furthermore, we also disagree with the statement that no empirical evidence supports our prediction: In fact, it uses an extensive data set based on 800+ multi-planet systems and on over 2,400 exoplanets, among other sources. This provides a very robust set of empirical data.

=================[ REFEREE'S COMMENT]========================
Sections 5 & 6:
These sections can be removed almost entirely because they offer the same information that can be found in Section 4.

-----------[ AUTHORS' RESPONSE]========================

We agree with the referee's comment that much of the information content in Sections 4, 5, and 6 was overlapping.  Therefore, we have adjusted the sections such that the Results section (Sections 4.1 and 4.2) shows only the specific outputs from our architecture analysis and temperature analysis, with the respective comparison to the previous analyses by Pepe+ 2011 and Feng+ 2017, as well as to the Solar System planet parameters, moved to their respective Discussion sections (Sections 5 and 6).

=================[ REFEREE'S COMMENT]========================
Section 7:
The authors explore how their claims could be used in future observations and they rightly identify a potential avenue in direct imaging. However, the discussion lacks the relevant details for observers to use their results. Direct imaging studies are performed at a specific wavelength where \lambda/D is used to identify the precision available to any particular telescope. The authors need to show what kind of telescope would be required (or cite the relevant publication) and at what wavelength to reach the necessary precision given the angular separation. Also, the authors need to show that the inner working angle does not obstruct the observations that the authors allude to.

-----------[ AUTHORS' RESPONSE]========================

We followed the referee's comment and expanded Section 7 with a more detailed discussion of the expected inner working angles of future telescopes. We also included a table that shows the minimum required mirror diameter (for two wavelengths) which will need to be combined with high-performance coronagraphs to image spatial separations that correspond to the orbits of the planets. 
As notable examples, we also show which planets would be detectable by two direct-imaging space mission concepts (LUVOIR and HabEx) and ground-based Extremely Large Telescopes. Finally, we also cited the relevant publications.

=================[ REFEREE'S COMMENT]========================
Section 8:
Due to the many issues outlined in the methodology and results, this section would need to be re-written. Otherwise many bullet points need to be removed (as outlined in the commented pdf).

-----------[ AUTHORS' RESPONSE]========================

We significantly revised Session 8 to reflect the changes that occurred in the manuscript.

=================[ REFEREE'S COMMENT]========================
A commented pdf is included for additional details

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for their extensive work in the review and the many comments provided in the pdf.  We have addressed all of the grammatical and syntactical issues brought to our attention. We followed most comments of editorial nature with a few exceptions.

=================[ REFEREE'S COMMENT]========================

By radius, the host star is more similar to a K dwarf.

-----------[ AUTHORS' RESPONSE]========================

We note that the radius of the star is 92\% that of the Sun, and taking into account its radius, mass, temperature, and luminosity, we find it to likely be a late G-type star.
Nevertheless, we now note in the manuscript the fact that some uncertainty remains on the spectral.

However, the spectral type itself is not relevant for our study: Our analysis is entirely based on physical parameters specifically determined for this star, and not on parameters that are typical to stars of a certain spectral type.

=================[ REFEREE'S COMMENT]========================

Instead of bullets, it is simpler to enumerate the hypotheses as a list with roman numerals or a scheme similar to Kipping et al. (2015).  This reduces the need to introduce a new nomenclature.

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for this suggestion but instead choose to keep our own nomenclature as we feel that it can be referred to more clearly. 

=================[ REFEREE'S COMMENT]========================
Figure 1
This shows that there is space available to potentially support a planet, not that it exists.  This is bordering on a Titius-Bode Law line of reasoning.

-----------[ AUTHORS' RESPONSE]========================

We note that the peaks in the orbital period likelihood are due to the probability distribution of orbital periods we assumed, and therefore are a prediction on the potential of a planet existing in that area of period space.

=================[ REFEREE'S COMMENT]========================

The peak for planet c indicates that there is space available for a planet.  One could have deduced an upper limit on planet c's mass using the dynamical spacing parameter without using DYNAMITE in a spreadsheet.  How much would this change depending on the assumption for delta_c in DYNAMITE?  Suppose you assumed a terrestrial planet-like spacing (Delta_c ~20), would the conclusions be the same?

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for this comment and note that an upper limit could be established for the mass of planet c using dynamical spacing alone. However, we use the mass range for planet c as given by previous analyses, since that is empirical evidence of its existence. 

Regarding the choice of Delta_c: The value we are using (Delta_c=8) is derived from  numerical stability experiments and it is a lower limit for the separations. We see no good reason to replace this lower limit with an average value (Delta_c=20) for the terrestrial planets. Corresponding, such a high value would be inconsistent with a large fraction of known multi-planet systems - we want to use the minimum limit for stability, not the average.

=================[ REFEREE'S COMMENT]========================

It is equally likely that the region is populated by asteroids or other small bodies.

-----------[ AUTHORS' RESPONSE]========================

We know of no evidence that would support the referee's statement; the relative likelihoods of asteroids belts vs planets has not been determined or constrained.
In contrast, extensive data sets exists for the occurrence rates of planets.
Our analysis relies on such datasets; therefore, we focus on the manuscript on planets and not asteroid belts.

Our statistics are focused on planets of moderate size (not minor bodies nor gas giants that could create asteroid belts), so the positions of high probability for these planets would likely mean a lower probability of minor bodies there.

=================[ REFEREE'S COMMENT]========================

This is a result of boundary conditions, where extrapolating planets for any system would always leads to a predicted planet in the author's framework due to the unconstrained nature of the problem.

This is also a result of boundary condition.  At least the previous set had some observational support, where this one has none.

-----------[ AUTHORS' RESPONSE]========================

We thank the referee for these comments and note that while there is less constraints on these predictions from the known planets in the system, these are still the most likely places to find an additional planet in the system, as determined from Kepler population statistics.
